Pitfalls in Experiments with DNN4SE: An Analysis of the State of the Practice

Software engineering techniques are increasingly relying on deep learning approaches to support many software engineering tasks, from bug triaging to code generation. To assess the efficacy of such techniques researchers typically perform controlled experiments. Conducting these experiments, however, is particularly challenging given the complexity of the space of variables involved, from specialized and intricate architectures and algorithms to a large number of training hyper-parameters and choices of evolving datasets, all compounded by how rapidly the machine learning technology is advancing, and the inherent sources of randomness in the training process. In this work we conduct a mapping study, examining 194 experiments with techniques that rely on deep neural networks appearing in 55 papers published in premier software engineering venues to provide a characterization of the state-of-the-practice, pinpointing experiments common trends and pitfalls. Our study reveals that most of the experiments, including those that have received ACM artifact badges, have fundamental limitations that raise doubts about the reliability of their findings. More specifically, we find: weak analyses to determine that there is a true relationship between independent and dependent variables (87% of the experiments); limited control over the space of DNN relevant variables, which can render a relationship between dependent variables and treatments that may not be causal but rather correlational (100% of the experiments); and lack of specificity in terms of what are the DNN variables and their values utilized in the experiments (86% of the experiments) to define the treatments being applied, which makes it unclear whether the techniques designed are the ones being assessed, or how the sources of extraneous variation are controlled. We provide some practical recommendations to address these limitations.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/Old_files/DNNs_old.tex <==

\section{Experimenting with Neural Networks}
\label{sec:NNexperiments}

%\sv{Take into consideration (ref. Bengio):

 %   \begin{itemize}
  %      \item The importance of changing benchmark dataset. We might end up having optimistic evaluations.
   %     \item In ML experiments, we often estimate the generalization error by computing the sample mean of the error on the test set. Algorithm A is better than B if the upper bound of the 95\% CI for the error of A is less than the lower bound of B. Bias vs. variance??
    %    \item The ideal network architecture for a task must be found via experimentation guided by monitoring the validation set error. Many NNs architectures have been developed for specific tasks (eg. convolutional).
    %\end{itemize}
    %}

%\se{@Sira: When reading this section I found it odd that we are defining the experiment types and designs without providing examples from the literature that we review, or better yet, a quantification of the how many of each type of papers we have accounted for in the last ICSEs, FSEs, etc. I see that we intend to do some of this on the next Section, but the separation between Section 3 and 4 is something that we need to reconsider because section 3 on its own is very dry and it does not make much sense without some examples. One idea is to have a section on What type of experiments are being carried out in Soft Eng with DNNs using our taxonomy, and the other on what experimental designs are being used/misused using our template. Each of these section would have at least two subsections, one defining our taxonomy/schema, and the other showing the state of the art} \sv{I agree that we should use the experiments we find in the literature (not the motivating example) to illustrate the concepts described here. But now I am unsure about the contents of this section. Should this be the Background now? Does it make sense to talk about experiment types now in this paper? According to the new structure, perhaps we could skip it. What do you think?}

%\se{Are you asking whether we need Section 3? I think we do. This is section where we can go deeper, where we start by defining DNN and the process to build them more carefully (as part current section 3.1), define the type of experiments and providea table quantifying how many of each we have seen, define the Design Space to Experiment with DNNs (as per Figure 1 -- I imagine part of our contribution would be a template where the user must determine whether a variable is manipulated, blocked, etc, and what values can/must it take). And then we can provide a table analyzing each paper from the previous section in terms of each of the variables as per the template. It is kind of an opportunity to zoom-in the results of the earlier table.} \sv{Yes, we do need it. I had a glitch.}



%\subsection{Neural Networks and Deep Learning}
%\label{sec:NNs}

%\sv{@Sebastian. NNs or DNNs? Now I am being inconsistent throughout the paper.}\se{Let's stick to DNNs from now on}

%\se{Should the background point to Fig2 to help with the description? It seems like a natural progression from left-to right, and a great visual walkthrough}
%\sv{Ok. Pending.}

%\se{This discussion is good, but I wonder whether we need to formalize it a bit, introducing the terms as variables that later on we can refer concisely when we defined our template. Something like the following (plagiarized from an older paper of mine  -- need to adjust). The key point is to introduce the terms that we will be using later in the other sections, like a domain-specific language or grammar for the domain}
%\sv{Ok. Pending.}

%\se{A DNN, N, is a type of machine learning model that is trained to approximate a partial target function $f : R_n \rightarrow R_m$. For example, f may classify some n-dimensional input (e.g., an image) as one of m possible classes (e.g., a digit in the range 0 to 9). f is partial in the sense that it is trained to generalize to a target data distribution, $D \in R_n$. 

%DNNs are comprised of layers, $l_0 , ..., l_k$ , each of which performs some computation on their input (e.g., matrix multiplication or convolution). A typical linear architecture defines a DNN as the composition of layers, $N = lk ◦···◦l1 ◦l0$. Layers are comprised of neurons. The input of a neuron is defined as the weighted sum of the outputs of a set of neurons in a preceding layer where the connections between neurons have trainable parameters. The output of a neuron applies a non-linear activation function to the input.

%Training involves initializing the parameters and then applying N to samples, (x, y), from the training set, T , and repeatedly updating parameters based on $\mid N(x)-y \mid$. The  goal of training is to learn the partial function f defined over D, D is generally unmanageably large (e.g., the set of road images visible on a forward facing camera). Consequently, the training set is defined as a representative sample of the data distribution, $T \sim D$. A well-trained network is said to generalize to the data distribution}


%Machine learning (ML) is a subfield of Artificial Intelligence (AI) that enables computers to learn from experience (ref. Mitchell, Bengio). ML algorithms build a model based on sample (training) data  to make predictions or decisions without being explicitly programmed to do so (ref?). Deep Learning (DL) is a specific kind of ML with Deep Neural networks (DNNs) (ref libro intro, Bengio). 

%\sv{Reducir.} NNs simulate the mechanism of learning in biological organisms (ref. NN\&DL). They consist of neurons, which are connected, and grouped in layers. There is always an input layer (that merely accepts inputs) and an output layer. Additionally, one or more \say{hidden} layers may exist between the input and output layer. A DNN has of two or more hidden layers, otherwise it is considered \say{shallow}. \sv{Quitar? In feedforward NNs, every neuron of a layer is connected to all neurons of the next layer, but neurons of the same layer are not interconnected.} Every connection between 2 neurons has a weight which regulates how much of the initial value will be forwarded to a given neuron. Each neuron has an associated value, called the \textit{bias}. 

%The output of a network is computed as the sum of the products of the inputs nd respective weights, plus the bias. Additionally, a nonlinear function (called activation function) can be applied to the logit. All neurons in the same layer must have the same activation functions, although different layers may have different ones. 

%This way, the flow of information goes from the first layer neurons, through the successive hidden layers to the output layer. A forward pass is the set of calculations that take place when the input travels through the NN to the output.

%NNs need to be trained before they can be used. \textbf{Training} a NN consists of (ref. Bengio) adjusting its \textit{parameters} (weights and biases), using a \textit{DL} algorithm controlled by a set of \textit{hyperparameters} (training and model), using a \textit{dataset}. It is performed via backpropagation---the reverse of a forward pass. The error the network makes when calculating the output is measured, and backpropagated using gradient descent\footnote{Gradient descent is a first-order iterative optimization algorithm for finding a local minimum of a differentiable function (ref.).} to modify the weights (and biases?) so that this error becomes very small. 

%\textbf{Datasets} are collections of examples (datapoints). Two types of datasets are used for training: training and validation (80\% and20\% of examples respectively \se{this is just a guideline, right? it is often different than that}) validation set test set. They are used to estimate the training error. If they are small, cross-validation is typically used\footnote{Repeat the training and testing computation on different randomly chosen subsets or splits of the original dataset.}. A test set is used to check how well the ML algorithm performs on data that it has not seen before. The test set is separate from training data, as it is intended to estimate the generalization error.

%\textbf{Hyperparameters} are parameters that cannot be learned: either because it is impossible \se{why?} or because they choose the maximum possible model capacity, resulting in overfitting. They can be classified as model hyperparameters (refer to the model selection task) and training hyperparameters, that in principle have no influence on the performance of the model but affect the speed and quality of the learning process (such as number of epochs, batch size or number of iterations).

%Nearly all \textbf{DL algorithms} can be described as a combination of (ref. Bengio): the specification of a dataset, a cost function, an optimization procedure and a model.

%A ML algorithm has a good performance if it makes: the training error small, and the gap between training and test error small. \textbf{Regularization} techniques are strategies explicitly designed to reduce the generalization (test) error, possibly at the expense of increased training error (ref. Bengio). These include: parameter norm penalties, dropout, data augmentation, early stopping, etc.

%\textbf{Optimization}. Finding the parameters (weights and biases) of a neural network that significantly reduce a cost function. Typically includes a loss function as well as additional regularization terms. Optimization is a extremely difficult task. Algorithms can be used, or parameter initialization strategies (no consensus of which one to use).

%\sv{Mention other architectures: Convolutional and recurrent. Others? Check with @Sebastian.}

%\subsection{Application of NNs to SE}

%\sv{Description of the types of problems being solved, and the form a typical DNN solution has (sometimes it is an end-to-end model, other times, different models are "composed", etc.)}

%\subsection{Experiment types}

%\se{If this is the only meaty portion left of Section 3, should we push it to section 2?} \sv{Makes sense. These are also findings. If I remember correctly, we decided to move the info out of Section 2 because it was too long. If you do not think that Section 2 will become again too long, I vote for moving it. But I have not read Section 2 yet.}

%\se{General question about categorization: what value is it providing to the reader? to the later analysis we do?}

%\se{Does it make to present the categories in terms of the space of variables they explore as per Fig 1? That would put Optimization experiments as exploring most of that space, Evaluation exploring the model parameters, etc.}



%Experiments are an essential tool in the context of NNs. They can be used not only when comparing different proposals, but also during their development~\cite{goodfellow2016deeplearning}. We have classified the experiments found in our literature survey according to their application \sv{goal?}: 





==> sections/Old_files/implications_old.tex <==

\section{Issues Found}
\label{sec:issues}

%\sv{@Sebastian, although I have worked on the section, it still needs to be improved. At this moment the list of threats is complete and they are in the correct place. But the writing in general (I think the messages, specifically problems and consequences) can still be made clearer to the reader, and also more examples need to be added.}

This section focuses on the most problematic aspects \sv{steps?} of Table~\ref{tab:state_practice}: variables identification, factors and treatments operationalization, design, analysis and interpretation, and validity evaluation. \sv{@Sebastian, I have finally decided to include a mini Section 3.5 to talk about them. We can decide later what we want to do with the contents.}


%\se{As per discussion on 7/28: focus on subset of key large issues and restructure them to first introduce the problem with an example, then the implication, then how it should be done, and close with recommendation} \sv{Done for sections 4.1 and 4.2.} 

For every aspect, we first describe it according to the experimentation literature. Next, we illustrate the problem(s) we have found in our literature review, using real examples. Then, we analyze how each problem affects the validity of experimental results, based on the classification developed by Shadish et al.~\cite{shadish2002experimental}: (statistical) conclusion validity (is there a relationship between dependent and independent variables?), internal validity (is the relationship causal?), construct validity (can we generalize to other concepts?) and external validity (can we generalize to other contexts?). Finally, we propose how the aspect should be addressed to avoid the problem by means of an example.  

\se{@SIRA: 8/11: BIG ONE TO DISCUSS: you are going to hate me, but I am having second thoughts about this section current organization. It reads as very "prescriptive", telling the reader a bit much on "how things should be done" without providing enough details of what is wrong  (even though  the examples are great they seem lost in the shuffle). And there is a some repetition (confounding seems to be key consequences across the sections, not surprise there). And it would seem more natural to see the Problem and Consequence of each example next to each other.  And we do not have much to recommend that is very insightful. One alternative would  be go back to four subsections with the four threats delineated above, providing 3 compelling examples for each (a mix of what is currently under problem and consequences), and then a big new table that makes a judgement on the ~50 experiment analyzed in terms of the threats that it affects them (rows being experiments, columns being general threat types). That would let us focus more on the impact of the under-specification described in the previous section. The drawback is that the connection to the steps in table-3 is much weaker, so somehow we would have to link the underspecification items from table 3 to the threats in this section}

%\se{throughout this section we use terms like "most" or "almost all" or similar ones that are NOT very useful at conveying the detailed study you have conducted. Instead, can we use a \% instead to be more precise?} \sv{@Sebastian, I have tried to fix this. Not sure if more numbers are needed. I still have to check that. Any suggestions?}
\clearpage

\subsection{Variables Identification}
\label{sec:variables_identification}

\textbf{Definition \sv{Description?}} The goal of this step is to identify all the variables that may influence the performance of a NN. These variables can be classified as either \textit{factors} (those subject of study in the experiment) or \textit{extraneous variables} (are not under investigation but may potentially affect the response variable and thus may influence results\footnote{Such potential influence often requires that it is controlled.}). Domain (NN) knowledge is required, which is typically a combination of practical experience and theoretical understanding~\cite{montgomery2019design}. \sv{@Sebastian, I think the following explanation can help reviewers to understand why we have created a step that is not used in ESE. Could be a footnote}. Note that this is not a separate step in empirical SE. Typically, factors are identified during its operationalization, and extraneous variables at design time. We have decided to separate it (along the lines of~\cite{montgomery2019design}) due to the higher-order complexity of the variables space in DNN experimentation, that affects not only the experiment context, but also the factors.

\se{@Sira 8/11: I am still unsure whether we can justify this separation of variable identification into its own step, and there is enough overlap with operationalization and design that I do not see the advantage of doing it differently from the usual process. Besides, this section is not as interesting as the other two...}


\textbf{Problem \sv{State of the practice?}} None of the papers from our literature review fully identify the variables intervening in their experiments. But some aspects show a better coverage than others. \sv{@Sebastian, not sure if the details are relevant.} Typically, training data is considerably well described (57\% of the papers fully describe it, being partially described by 85\% of the papers). Model hyperparameters, training hyperparemeters and DL algoritm are never fully addressed, but partially in most of the papers (85\%, 83\% and 91\% respectively). Model parameters are poorly addressed (missing in 78\% of the experiments). 

%\se{It would be nice to have a few examples here from a handful of papers each missing something different} 
Note, however, that a \textit{partial} identification of variables ranges from a poor (very few variables are identified) to a good (but incomplete) one. For example, paper (ref. paper 26) fully describes model parameters and training data. As regards the DL algorithm and the training hyperparameters, it only misses the regularization term and the number of iterations respectively. However, model parameters are very loosely described (no parameters initialization is reported, activation functions and number of neurons are mentioned for some layers only, and it is not clear the number of layers. \sv{@Sebastian, not sure if this is the type of examples you wanted. It consumes too much space. Perhaps we can omit the details about which specific variables are missing? This way we could include more papers in the same example.}\se{I think we should keep these examples as they are the main way we have to concretize the issues we are bringing up, otherwise this could be a paper about experiments with any experiment} On the hand, paper (ref. paper 60) provides no description of the model parameters and hyperparameters, the training data is partially described, and only half of the variables corresponding to the DL algorithm and training hyperparemeters are reported. \sv{One of the FSE papers that I have just read is even worse than this. Check and replace if necessary.}


\textbf{Consequences \sv{Implications?}} Not accounting for all the variables involved in an experiment may have different consequences depending on whether the omitted variables are part of the definition of factor or extraneous variables. The construct and internal validity of the experiment will be compromised, respectively, with the following threats:

\begin{itemize}

    \item\textit{Inexact definition of constructs (construct underrepresentation)}. Failure to completely define a construct may lead to incorrect inferences about the relationship between operation and construct. This happens in evaluation experiments, since the NNs they use are not comprehensively described in terms of the variables represented in Figure~\ref{fig:fishbone}. For example, in (ref. paper 26), the authors do not report the regularization term, the number of iterations and the topology of the proposed NN. Therefore, in the case it performs better, they cannot claim that their proposal is better, as a NN without these variables being defined is not functional. \sv{@Sebastian, I need to improve this. I mean that all these variables need to be set in order to be able to "run" the NN. Therefore, it is impossible that what you have described can be better than any other thing, because it cannot even be run.}
    
    \item \textit{Confounding}. Changes in the dependent variable may rather be attributed to variations in a third variable which is related to the manipulated variable. For example, none of the optimization experiments acknowledge random initialization of model parameters as a confounder, but it is. For example, in the optimization experiment reported in (ref. paper 30), Xavier initialization of parameters is used, and the factors are: regularization, number of hidden layers and learning rate. However, since the confounder is not acknowledged it is not possible to know if the best configuration is due to the combination of levels of factors or just a fortuitous (random) selection of parameters.
    
\end{itemize}


\textbf{Proposed solution \sv{Practical recommendation?}} We propose to start with a systematic evaluation of the variables in Figure~\ref{fig:fishbone}, so that, for each one, a decision is made on whether it is a factor (or part of a factor) or an extraneous variable in your experiment. Additionally, we suggest to explore the existence of other variables that could potentially be influencing the performance of the NN in your experiment. \sv{@Sebastian, I can think of setting variables. e.g. having two computers with different hardware and you want to use both for your experiment. But perhaps it is a crazy example... should I use a real one instead?}


\begin{comment}
\noindent\framebox{%
\begin{minipage}{0.97\linewidth}
\textbf{Practical recommendation:} \newline
Variables intervening in the experiment must be accounted for. Domain (NN) knowledge is required to do this. Figure~\ref{fig:fishbone} can be used for this purpose.
\end{minipage}}
\end{comment}


\subsection{Factors and Treatments Operationalization}
\label{sec:operationalization}

\textbf{Definition \sv{Description?}} This step involves choosing the experiment factors along with their treatments. As an example, the NN is the factor in experiments categorized as Evaluation (being the treatments the different NNs examined), while hyperparameters could be the factors in the  experiments of the Optimization category (being the treatments the range of values examined for each hyperparemeter). Their operationalization implies describing them in terms of their prototypical features\footnote{Those characteristics that are appropriate and relevant for the goal of the experiment.}. 
%However, deciding which features are prototypical is a difficult task. It depends on the context on which the factors are to be used (i.e. the experiment goal). 


\textbf{Problem.} Almost all experiments (98\%) in our literature review do not fully operationalize their factors and treatments. It is a direct consequence of not having properly identified the variables involved in the experiment (as described in Section~\ref{sec:variables_identification}), which is causing that the features used for description are not the prototypical ones. \se{what do we mean by prototypical?} \sv{See if footnote in previous paragraph is enough.}

Additionally, none of the evaluation experiments operationalize the state-of-the-art NNs that are used for comparison against the proposed one. In most of the cases (83\%) a mere reference to the paper where they are proposed is given, complemented in some cases with an explanation on how their performance results have been obtained (either from the original paper where the state-of-the-art NN is described, running the code provided in the original paper, or running a new implementation of the NN). For example, in (ref. paper 5) the authors compare their approach \sv{Should I give names?} against three other state-of-the-art approaches. For one of them, they use the stable version available in Github. For another, they implement the approach following the original paper where it is proposed, and for the last one, they use the numbers reported in the paper where it is originally proposed.\se{So they are comparing their approach against 3 treatments obtained through different means -- but why is that problematic if they are well defined?}

In the case of optimization experiments, most of them (78\%) are hidden, meaning that factors and/or levels could be missing. The cases of experiments fully addressing the operationalization of factors and treatments correspond to this type of experiments \se{Optimization? but I thought most of them are missing?}. For example, in (ref. paper 60), it is specified that the factors are: Word2vec vector length (with values 100, 50, 120), learning rate (with values 0.001, 0.005, 0.01) and epoch size  (with values 100, 200, 300).\se{Ok, so this last one is a good example among all the bad ones? I was not sure }

\textbf{Consequences \sv{Implications?}} ) Failure to properly undertake the operationalization of factors and treatments will threaten the construct \se{undefined?} validity of the experiment~\cite{shadish2002experimental}. More precisely, the following threats:

\begin{itemize}

    \item\textit{Construct confounding (extraneous construct content)}. Operations usually involve more than one construct, and failure to describe all the constructs may result in incomplete construct inferences. For example, in the comparison experiment reported in (ref. paper 59), the prototypical feature used to define the construct is the NN architecture (deep adaptation networks versus deep belief networks versus LSTM versus CNN). However, it is impossible to know whether the architecture is the factor causing the performance gain or whether other non-specified variables like the DL algorithm or the data representation are the underlying causes.
    
%    \item\textit{Construct confounding}. Operations usually involve more than one construct, and failure to describe all the constructs may result in incomplete construct inferences. In the above example on evaluation of a given approach versus other state-of-the-art, the characteristic used to define the construct is \say{the type of information used to infer the function's type signature}

    \item\textit{Confounding constructs with levels of constructs}. Inferences about the constructs that best represent study operations may fail to describe the limited levels of the construct that were actually studied. For example, in (ref. paper 27), the performance of the authors' proposal is compared against state-of-the-art ones. But it is not possible to assess if the observed results hold for other training hyper-parameters than the concrete values chosen for this single experiment. In this context, it would not be \say{fair} to use the NN topology as a description for your treatments because you only looked at a single value for training hyperparemeters\footnote{To conclude that the NN topology is the best you should try with a relevant number of different training hyperparemeters}. \sv{@Sebastian, not sure if I managed to show that both threats are different...}\se{Both are good examples, I just could not tell the difference by type}
    
%    \item\textit{Unreliability of treatment implementation}. If a treatment that is intended to be implemented in a standardized manner is implemented only partially for some respondents, effects may be understimated compared with full implementation.
    
\end{itemize}

%\sv{@Sebastian, probably this is too advanced. Not sure if it could be interesting for ICSE. Besides, it is not critical, just something that should be kept in mind.} \se{I am not sure. It does not seem complicated but it seems less lethal than the other as it mainly restricts the scope of the claims.The question is whether this is an issue that you have seen often enough in the papers that is worth mentioning. If it is, we should consider adding it. } \sv{All papers suffer from this. No-one has implemented the same NN in two different ways. I would classify this type of threat of something you should be aware of. To me, it is the same type of advice that we gave for the response variable. To be consistent, I would save it for the future. Discuss in the next meeting???} Additionally, there is a threat that, although not critical, is worth to be mentioned. It is the \textit{mono-operation bias}. Any one operationalization of a construct both under-represents the construct of interest and measures irrelevant constructs\se{Why/How does it measure irrelevant constructs?}, \sv{Added to next sentence.} complicating inference. If you only use a single implementation of a NN in a single computer, you may not be capturing the full breadth of the concept of the NN \se{True, more is better, but how many do you need to claim breath? Again, this is a softer issue than the others }, and may be incorporating the implementation details into the construct. It could be argued that the results of your study only reflect that particular version of the NN that you implemented, and not the actual construct you had in mind. The solution in this case would be to try to implement multiple versions of your NN.

It is important to note that these validity threats are essentially related to the description of your factor and treatments. The description you are providing is not a good one for what you are experimenting with.

\textbf{Proposed solution.} Identify, from the set of variables in Figure~\ref{fig:fishbone} which ones are part of the experiment factors, and define their values. For example:

\begin{itemize}
 
    \item In the optimization experiment performed in (ref. paper 3)\footnote{This is a hidden experiment, and its information has been deduced from the paper.}, the factors appear to be: number of convolutional layers, number of convolutional layers filters, number of hidden states in the recurrent layer and beam size. Therefore, the prototypical features of the constructs would correspond to single variables in Figure~\ref{fig:fishbone}, and the treatments would correspond to the specific values chosen for each variable.
    
    \item In the evaluation experiment performed in (ref. paper 22), the factor is the NN (being the treatments different state-of-the-art approaches). In this case, the prototypical features of the construct would correspond to all variables that appear in Figure~\ref{fig:fishbone}, and the treatments would correspond to the specific values chosen for the whole set of variables for each NN.
    
    \item In the generalization experiment performed in (ref. paper 23), the factor is the dataset. In this case, the prototypical features of the construct would correspond to the variables in the \textit{dataset} rib of Figure~\ref{fig:fishbone}, being the treatments the specific values chosen for the variables in the rib for every dataset.  

\end{itemize}



\begin{comment}

\noindent\framebox{%
\begin{minipage}{0.97\linewidth}
\textbf{Practical recommendation:} \newline
Factors and their treatments need to be properly described, to avoid construct validity issues. We propose to identify the variables from Figure~\ref{fig:fishbone} that are part of the experiment factors, and define their values.
\end{minipage}}

\end{comment}


\clearpage

\subsection{Design}
\label{sec:design}

\textbf{Definition.} Ideally, the only source of variation in an experiment should be the one due to the manipulated variables (factors). In practice, there is variation (experimental error) among identically and independently trained NNs. There are two types of error: systematic (confounding) and random (error variance). Generally, we want to minimize random error, and eliminate systematic error. Experimental error can be addressed by means of the three fundamental components of experimental design~\cite{kuehl2000design}: local control (noise reduction), randomization and replication. The two first address systematic error, while the latter addresses random error.
%\textit{Local control} describes the actions an investigator employs to reduce or control experimental error, and therefore increase the accuracy of observations.
%Such actions include 1) the definition of an experimental protocol to guarantee that experimental tasks are performed uniformly throughout the experiment~\cite{kuehl2000design}, 2) the selection of experimental units that are as uniform as possible~\cite{kuehl2000design}, 3) the management of other variables by holding them constant, block them and measure them~\cite{montgomery2019design}, and 4) the design selection to assign treatments to units 	\cite{wohlin2012experimentation}. Local control: 
%	\begin{itemize}
%		\item Experimental protocol:  Steps for \textit{running} the code.
%		\item Selection of experimental units: These are the runs (entity which can be assigned, at random, to a treatment; entity a researcher wants to make inferences about and for which adequate replication is needed)
%		\item Variables control: Which variables are held constant. Not sure there are blocking variables or measured covariates here.
%		\item Experimental design: Complex ones in terms of number of factors and levels (compared to human-based experiments). Typically factorial and fractional factorial designs. Maybe also nested designs.
%	\end{itemize}
%\textit{Replication} is an independent repeat run of each factor combination~\cite{montgomery2019design} to estimate the experimental error variance and allows a more precise estimate of the population mean~\cite{kuehl2000design}.
%Replication has two important properties: (1) It allows the experimenter to obtain an estimate of the experimental error (and it becomes a basic unit of measurement for determining whether observed differences in the data are really statistically different); (2) if the sample mean is used to estimate the true mean response for one of the factor levels in the experiment, replication permits the experiment to obtain a more precise estimate of this parameter. The practical implication of this is that if we had 1 replicate, we would probably be unable to make satisfactory inferences about the effect of the treatment. That is, the observed difference could be the result of experimental error. Several runs are needed.
%\textit{Randomization} is the random assignment of treatments to experiments units that allows a valid estimation of experimental error variance\footnote{It removes biases that arise through sytematic assignment of treatments to experimental units. Eg. \sv{An example}}.
%Used for uncontrolled variables for which we assume relatively small effects~\cite{montgomery2019design} or that are unknown (ref. libro observational studies). Explain why this does not apply to this type of experiments. \se{I am confused. Isn't randomization a key piece of the design as units are assigned to treatments? Isn't a way to control error (not estimate it)?} \sv{Not exactly. It is a way to make that the part of the error that you cannot control is not biased. The underlying assumption is that there is part of the error that cannot be controlled (cannot be addressed in local control step), and all you can hope is that it is not biased. Note that you are supposed to use randomization for unknown variables or variables with very little influence (otherwise local control techniques should be used instead).}\se{I understand the response and agree wit hit, but I just do not understand the wording in the first sentence of the text "valid estimation of experimental error variance"}
These are applied in the tasks that are performed when designing an experiment: choice of design (describes how the series of tests of the treatments that it is composed of are organized and run) and instrumentation (provides means for performing the experiment and to monitor it) \cite{wohlin2012experimentation}. 
%

%according to Table~\ref{tab:dealing_extraneous}. 
\begin{comment}
\begin{table}[h]
  \caption{Extraneous variables and how to deal with them}
  \label{tab:dealing_extraneous}
%  \small
  \begin{tabular}{llll}
  \toprule
	\multicolumn{3}{c}{\textbf{Characteristics}} & \textbf{How to treat}  \\
	\textbf{Known} & \textbf{Controllable} & \textbf{Measurable} & \\
	\midrule
	Yes & Yes & N/A & Held-constant \\
	Yes & Moderately & N/A & Blocking \\
	Yes & No & Yes & ANCOVA \\
	No & N/A & N/A &  Randomization \\
\bottomrule
\end{tabular}
\end{table}


\end{comment}


\textbf{Problem.} None of the experiments surveyed include the choice of design \se{This seems waaayyy too strong. Are we setting the bar too high? Are some partially defined designs alsmost there? } . We could not find extraneous variables explicitly controlled \se{Are they perhaps explicitly controlled but perhaps not explicited stated that they are controlled?} in the experiments we have reviewed, although we have deduced that they sometimes exist. This would be the case of the dataset in experiments where multiple are used (ref. paper 58, 60), version in the experiments reported in (ref. paper 59), where multiple versions of programs are used, or project in the experiments reported in (ref. paper 62), where multiple programs are used. Additionally the number of replications is never reported (although we have deduced that no replication is performed, as only one run of the NN for each dataset is reported). The experimental objects (test sets) are very often described (79\%), and the experimental protocol (how the response variable will be measured) is always partially addressed. \sv{Add examples.}

\textbf{Consequences.} The unique strength of controlled experiments is its internal validity (causality) due to its ability to link cause and effect through treatment manipulation, while controlling for the spurious effect of extraneous variables. Failure to properly design an experiment will threaten its internal and  conclusion validity:

\begin{itemize}

    \item \textit{Confounding}. Changes in the response variable may rather be attributed to variations in a third variable which is related to the manipulated variable. For example, in paper (ref. paper 62), the program is an extraneous variable that has been left "uncontrolled". This means that it is impossible to know if the results reported are due to the proposed approach or simply that the proposed approach works better with these specific programs.

    \item \textit{Low statistical power}. An insufficient powered experiment may incorrectly conclude that the relationship between treatment and outcome is not significant. It is necessary to set a high enough number of replications (this issue is discussed in \cite{arcuri2011practical}). All our papers are an extreme situation of low statistical power, as they work with just one replication. For example, \sv{Complete}.

\end{itemize}

\textbf{Proposed solution.} We propose to perform the required tasks (The first two correspond to the choice of design and the last two to the instrumentation): \sv{@Sebastian, not sure what type of experiment should I use as a starting point for for this example.}

\begin{enumerate}

    \item Decide the number of replications to be performed. There are different sources of random error in NNs. They are due to different sources of non-determinism including parameter initialization, data shuffling, data augmentation, stochastic regularization and low-level operations among others~\cite{summers2021nondeterminism}. A typical value in experimentation is run 30 replication. 

    \item Deal with extraneous variables. These should have already been identified, as explained in Section~\ref{sec:variables_identification}. For every variable it is necessary to decide how it will be controlled. The mechanisms used in experimentation for this are: randomization, blocking, held the variable constant, or leave it uncontrolled but measure it.

    \item Selection of experimental objects. Defined the test set(s) that will be used.

    \item How the response variable is going to be measured. This includes making explicit the instruments that will be used to measure it and the protocol that will be followed to measure it.

\end{enumerate}

%\clearpage


\subsection{Analysis and Interpretation}

\textbf{Definition.} Statistical analysis is \say{any of a wide range of techniques used to describe, explore, understand, explain, predict, and test hypotheses about data}~\cite{apa2007dictionary}. It involves using procedures for summarizing sample data, without inferring to a larger population (\textit{descriptive statistics}) and probabilistic models that allow inferences about a population from its sample, while partially controlling the extent to which errors of inference may be made (\textit{inferential statistics})~\cite{apa2007dictionary}. Statistical methods and experimental design were two sides of the same coin for Fisher~\cite{fisher1973statistical}. The reason being that when an experiment involves data that are subject to experimental errors, statistical methods are the only objective approach to analysis~\cite{montgomery2019design}. This is the case for NNs experiments, as we have discussed in Section~\ref{sec:design}.

\textbf{Problem.} As Table~\ref{tab:state_practice} shows, more than half (63\%) \se{\%, and what they usually have ? plots? how many, etc?} \sv{Nothing. If they completely miss it, it means they have nothing.} of the experiments in our literature survey completely miss data analysis, while none of them fully address it. Typically, the only descriptive statistic reported for the response variables is the mean, being the standard deviation scarcely reported (3\%). Graphics are used as a means to report the raw data. Diagrams such as box-plots are only used in less than 1\% of the experiments. The few experiments (7\%) that perform inferential statistics use non-parametric tests without having checked if parametric tests could have been used\footnote{At least, they do not report having checked it.}. Furthermore, since the experimental design is not properly described, there is no way to know if the statistical test used is the appropriate one. No measures of effect size are reported (although mean difference could be computed by the reader when the means are reported).

\textbf{Consequences.} Failure to statistically analyze the data gathered from an experiment will threaten its (statistical) conclusion validity. This means that valid inferences about the existence and size of a relationship between the factors and the response variables cannot be drawn~\cite{shadish2002experimental}. The observed differences in results can perfectly be due to random error rather than the factors. For example, in paper (ref. paper 9), the authors conclude that the best option is a typed-tree model (versus typed-simple), with values for the response variables F1, AUC and Kruskal's \textgamma respectively of 0.931 (0.920), 0.991 (0.988) and  0.992 (0.989). Note that a mere standard deviation of 0.0055, 0.0015 and 0.0015 in the response variables will invalidate the conclusions. \sv{Mejorar la explicacion.}\se{That is an awesome example!!!} \sv{@Sebastian, there are no examples so far for the problem of incorrectly using box-plots for inference. There are only 5 papers reporting box-plots, and they are correctly used (in 3 of them statistical analyses are reported, and in the other 2 cases, the box-plot is used to show the distribution of values, not inference).}\se{Maybe that is worth saying, that the papers that introduce them use them well}
    
%\se{The following seems generic and not as relevant given that most paper did not even perform a statistical analysis. I would rather put the focus on emphasizing the problem and consequences of having just means, or having just box-plots which is what we see in the best case} \sv{@Sebastian, I have removed the detailed listing of applicable validity threats according to your suggestion. Not sure if you also want to remove this paragraph. I think it is relevant, as we are highlighting that people still do not pay attention to issues that have been raised by other authors, and they have proposed how to address them. My feeling is that if we just stick to the issues related to lack of analysis, in the next "generation" of papers we will see a lot papers that are not properly analyzed.} 
But even those experiments that perform data analysis may threat conclusion validity. They suffer from the same issues already reported in~\cite{reyes2018statistical}, as they do not follow established guidelines, such as~\cite{arcuri2011practical}. \se{Maybe add a bit about each, what part are the authors missing and why it matters again.}

\textbf{Proposed solution.} We suggest to follow common recommendations in empirical SE~\cite{juristo2013basics,wohlin2012experimentation}. \sv{add references to: Lionel ICSE 2011, Óscar ICSE 2018, guidelines Andreas, my ICSE tutorial?}. For example, the analysis of the results reported in the evaluation experiment in (ref. 59) would look like: \sv{@Sebastian, too long.}


\begin{enumerate}

    \item \textit{Report descriptive statistics}. This includes the description of measures of central tendency (mean, median and/or mode) and dispersion (range, interquartile range, variance, and/or standard deviation). Additionally, graphical representations (such as box-plots) should be used. Table~\ref{tab:descriptive_statistics} shows the descriptive statistics for our experiment, and Figure~\ref{fig:boxplot} shows the corresponding box-plot.
    \se{Are those from one of the papers we analyzed that did a good job?}
    
\begin{table}[h]
  \caption{Descriptive statistics}
  \label{tab:descriptive_statistics}
  \small
  \begin{tabular}{lccccccc}
  \toprule
	&	\textbf{N}	&	\textbf{Mean}	&	\textbf{Std.}	&	\multicolumn{2}{c}{\textbf{Mean 95\% CI}}	&	\textbf{Min.}	&	\textbf{Max.}	\\  \cmidrule{5-6}
	&		&		&	\textbf{Dev.}	&	\textbf{Lower} 	&	\textbf{Upper}	&		&		\\ \midrule
	
\textbf{DBN-CP}	&	22	&	56.75	&	15.10	&	50.06	&	63.44	&	31.6	&	97.9	\\
\textbf{TCA+}	&	22	&	47.94	&	10.96	&	43.08	&	52.80	&	29.2	&	65.1	\\
\textbf{DP-LSTM}	&	22	&	49.45	&	17.85	&	41.54	&	57.36	&	26.1	&	78.5	\\
\textbf{DP-CNN}	&	22	&	52.82	&	10.56	&	48.14	&	57.50	&	32.3	&	67.1	\\
\textbf{DTL-DP}	&	22	&	61.75	&	14.53	&	55.31	&	68.19	&	39.5	&	82.7	\\ \midrule
\textbf{Total}	&	110	&	53.74	&	14.70	&	50.96	&	56.52	&	26.1	&	97.9	\\
  
\bottomrule
\end{tabular}
\end{table}
    
    \begin{figure}[h]
      \centering
      \includegraphics[width=\linewidth]{figures/boxplot.jpg}
      \caption{Box-plot.}
      \label{fig:boxplot} 	
    \end{figure}

    
    \item \textit{Write your statistical hypotheses}. Both null and alternative(s). They would read:
    
    H0: There is no difference in performance between the different approaches examined.
    
    H1: Not all approaches examined behave equally in terms of performance.
    
    \item \textit{Perform inferential statistics}. Select the most appropriate statistical test, based on your design. Check if data meet its assumptions. Otherwise, use data transformation or non-parametric tests. For a good description of statistical tests, see~\cite{field2017discovering,field2012discovering}. \sv{Mention Bayesian statistics as an alternative to the classical approach of NHST.}
    
    In this case, we do not have information about the experimental design. Therefore, we will assume that we have a 1-factor-5 levels experiment. The most appropriate statistical test in this situation is the 1-way ANOVA. Both the normality and homogeneity of variances assumptions are met (the results of the Shapiro-Wilk test for each approach are 0.30, 0.05, 0.07, 0.22 and 0.14, and the result of the Levene test based on means is 0.06). And the results of the 1-way ANOVA show that we can reject the null hypothesis (p=0.01). The Tukey multiple comparison tests show that the proposed approach (DTL-DP) shows a better performance than TCA+ and DP-LSTM, but its performance is similar to DBN-CP and DP-CNN~\footnote{This contrasts with the conclusions of the paper about DTL-DP showing the best performance.}.

    
    and homogeneity of variances requirements are met. T
    
    \item \textit{Measure effect size}. Report appropriate measures for effect size along with their confidence intervals. For a good description of effect sizes see~\cite{ellis2005effectsizes,grissom2005effectsizes}. \sv{Pending.}
    
\end{enumerate}

\subsection{Validity Evaluation}

\sv{Not sure what to do with validity threats. I have the feeling that it is the typical section that authors know they have to fill in, but do not consider relevant, and therefore they try to do the minimum. I do not think it is very constructive to say people "take the listings in the Shadish book and go one by one deciding if it affects your experiment". And most of the times the missing parts are due to the other issues found (lack of design, not proper operationalization...). Probably we can just say something in the line of the next sentence.}\se{Maybe one reason not to cover it is that it is not specific to the domain of DNNs right? it seems more general and hence not worth focusing on it} \sv{I have been thinking a little bit more about this, and now I think that it is the other way round. The current list of validity threats is not specific for this type of experiments, and researchers find it difficult to identify the validity threats that are affecting their study. The solution would be to develop a specific list of validity threats. But still I am not sure if it is interesting enough to be covered.}

\sv{@Sebastian, very draft, as at this point I am not sure if it makes sense to include this issue in the paper, and if so, how much in depth.}

\textbf{Definition.} The goal of this step is to assess the extent to which the results of the experiment accurately correspond to reality~\cite{shadish2002experimental}. Note that the validity judgements of an experiment are not absolute; It is more a matter of degree than of existence or not.

\textbf{Problem.} None of the experiments in our literature survey properly address the validity evaluation step \se{What would it mean do it properly? Where is the bar?}. For the simple reason that there is no single paper that does address all validity threats we have covered in this paper. Furthermore, 33\% of the experiments we have surveyed do completely lack from an assessment of their validity. For those that do a partial assessment, X\% merely list some validity threats without linking them to any of the four categories. For example, in (ref. paper 26), only 3 validity threats are listed, while in (ref. paper 27) only 2 validity threats are listed. In both cases, they are not linked to any category. Only Y\% experiments link them to their corresponding category. But even in these experiments, the main focus are the internal and external validity threats. Conclusion validity threats are never mentioned, and construct validity threats (discussed in only X\% of the experiments) are evaluated for the response variable only (never for factors and treatments). Finally, in all cases, the validity evaluation is not made individually for each experiment, but at the paper level.

\textbf{Consequences.} The validity of an experiment is synonym with its quality. An improper evaluation of the validity threats of an experiment will create a biased perception of its quality.

\textbf{Proposed solution.} Currently, the only set of validity threats instantiated for experiments with NNs is the one presented in this paper \sv{@Sebastian, which is incomplete}. Consider how these threats affect your experiment, as they are the most critical. Think if there are other threats that could be affecting it. A good starting point are~\cite{shadish2002experimental,wohlin2012experimentation}. \sv{Add example if we finally decide to include it in the paper.}

\sv{I think a (nice, at least to me) "side" contribution of this research is provide researchers with a list of validity threats instantiated for NNs experiments. But remember that it is incomplete, as there are more threats that we are not including here that although not "critical" should be taken into consideration.} 

\se{I agree that would be a nice contribution: do we have an initial list?}


==> sections/Old_files/introduction-old.tex <==

\section{Introduction}
\label{sec:intro}

The application of deep learning (DL)
%\sv{Shall we define the acronym here (DL) and use it throughout the paper instead of the full term?} 
techniques across the software development life cycle is becoming a thriving  research thread in the software engineering (SE) community. Such emerging techniques, often grouped under labels such as  DL4SE or DNN4SE,
%\se{maybe generalize the term from DNN4SE to ML4SE?}\sv{Not sure. The paper is about DNN4SE. If we generalize here, then we have to specify later that the paper focuses on DNN4SE} 
have rendered promising results  supporting the automation of activities ranging from  requirements engineering to code maintenance \cite{SE4DLreport}. 
Similar to other DL application areas, the maturation of frameworks and tools that lowered the adoption for such technology has facilitated their application in the SE domain. In addition, our community is in an advantageous position in that we can tap into a continuously increasing number of public repositories with various types of software artifacts such as code and tests  that constitute rich data sets on which DL techniques can thrive.

%\se{@Sira: I changed this paragraph quite a bit. The example was useful to write it, but in the end I could not find a way to use it effectively. Take a close look at it to make sure it convinces you (and hopefully the reader) that this is a hard problem} 
To assess such techniques, researchers  perform   experiments in which variables are manipulated in a controlled environment to investigate their impact  over response variables~\cite{juristo2013basics}. Conducting such experiments, however, can be extremely challenging given the number and complexity of variables that may affect a technique that relies on DL.  %\se{Point from Sira: make sure we emphasize that the space of variables is large and complex, and that we will elaborate on that in section 2.} 
Tens of variables play a fundamental role in how a deep neural network (DNN) is set up as part of an experiment. 
Some of these variables are inherently complex as they point to  optimization procedures that contain their own set of parameters. Other variables
like those associated with  datasets or competing models often point to online resources that  may unsuspectingly evolve.
%potentially rendering suspect comparisons. 
Other variables, like the  sample size used by gradient descent to set the network weights or the proportions of data used for training and testing, are deceptive simple, yet they constitute  sources of randomness 
%as to what samples are used which
that will impact the   DNN's performance.  
Yet other variables that may not be explicitly defined, like the ones defining termination criteria, can have subtle interactions with other variables undermining the implementation of the intended experimental constructs.
%that if left unidentified may implement constructs that are different from the intended ones. 
%\sv{I think we should add an example here. It is hard to find one. I think sometimes unidentified variables means no value or using defaults. E.g. regularization (if not mentioned, probably means none used) or initialization of parameters (empty means random?). But defaults might change in the future, and no values could be that you forgot to mention the value of the variable.}
%(see Figure~\ref{fig:fishbone}\footnote{Excluding variables related to the DNN´s technological environment.}). 
%Some of these variables have single values (e.g. batch size, loss function), others are optional (e.g. regularization), but others may have a number of values that depends on the size of the DNN (model hyperparameter variables). 
%The difficulties in setting the appropriate values for all those variables are exacerbated by their hard to tease dependencies. To top it off, there are several sources of randomness in the training process used by these techniques that add further challenges in exercising  control during the experiment.
%For example, consider the DNN proposed in~\citeAP{paper22}. Although it is a simple one (it has 3 layers: input with 100 neurons, bi-directional LSTM with 512 neurons and output with 978 neurons), there are thousands of variables involved in it. \se{we need sample from one of the papers we analyzed, it would be nice to have a simple one in terms of technique, so that we can focus on enumerating the factors} \sv{I am not sure if this is what you wanted}
When evaluating the application of a DL technique to an problem through an experiment, the lack of careful consideration of such variables can  dramatically impact the findings. 




%Following with~\citeAP{paper22}, the paper does not account for the activation functions used, how the weights and biases have been initialized, the learning rate used, how extraneous experimental variables have been addressed in the experimental design, if the DNNs involved in the experiments have been trained more than once to address randomness, or how the state-of-the-art DNN it is compared to (DeepTyper) has been trained and whether modifications to its publicly available artifact have been made\footnote{The paper neither contains this information, nor points to where it could be found.}. 

%\se{keep going with the previous sample paper enumerating the potential weaknesses because the factors are not accounted for} \sv{Same. Not sure if this is what you wanted.}

%\se{@Sira: I changed the argument a bit in this paragraph to hopefully make it stronger and better connected to the findings. Take a very critical look}
We are not the first community facing this challenge. The artificial intelligence community has developed various checklists to mitigate common experimental pitfalls~\cite{AAAI2023checklist,ML2020checklist,NeurIPS2022checklist}.
%\sv{Should we reference AAAI and NeurIPS guidelines? They are based on the one we reference. The problem is that they are getting closer to what we claim...} \se{Yes, please cite all them. Please add. Then we will tweak the following given those} \sv{Done}
We  support the thoughtful adoption of similar practices by the SE community. However, it is unclear whether existing checklists would  address the most pressing challenges for the SE  community which is why characterizing the state-of-the-practice as we are doing is crucial. As we shall see, for example, we find that such checklists may improve the reproducibility of the results, but they would be unlikely to provide more insights into key experimental decisions made like the choice for experimental design  to control noise and the analysis to identify meaningful relationships in the SE context. 
%For example, a perfectly reproducible package may tell us what values were set for all variables but not ... \se{complete thought here?}
%\se{@Sira: After fresh read: Not sure the last line is convincing yet. Is the design rational missing? If they can reproduce it, what are they missing?} \sv{This could be a philosophical issue. They want you to have all the code, data, etc. so that you hit the key and get exactly the same results. This a first step, definitely challenging in this type of systems. But, as the saying says "You can not expect a new result if you keep doing the same thing". In other fields (does not happen in SE), researchers use the description of the experiment to challenge it and improve it. We should aim higher. Not only wanting to be able to reproduce the results, but also knowing how the experiments have been conducted so that researchers can replicate it making as many changing as they wish. For this, the code is definitely needed, but it is not enough.}. 
Similarly, the SE community has developed an extensive body of knowledge~\cite{arcuri2011practical,jedlitschka2008reporting,jorgensen2016incorrect,juristo2013basics,ralph2020guidelines,wohlin2012experimentation}  
to improve the quality of the experiments we conduct (Section~\ref{sec:related_work} provides further details). As part of that body of knowledge, existing guidelines are naturally relevant and applicable to experiments conducted in the DNN4SE domain. However, as it shall become clear from our findings, there is a distinct and urgent need for the community to become much more cognizant of the space of variables particular to the DL domain.
%to properly design and implement experiments on DNN4SE. 

%{\color{violet}This paper aims to answer the following research questions:}

%\sv{@SE: If we are not going to have a final paragraph in the intro explaining the contents of the paper we need to reference in each RQ the section where it will be covered (now included in the file, but commented).}

%\se{@Sira: I did not think the questions fit well before contributions because it was odd that they were not mapped to the particular contributions in the following paragraphs, so I integrated them in the following paragraphs with references to the proper sections. Check if it works} \sv{Seems ok to me. The only (cosmetic) issue is that it might seem weird that not all sections are mentioned here, and there is a gap in sections between contributions 3 and 4.}

\se{Missing transition / check comment from Sira about structure of paper in sections}

\vspace{0.05in}  \noindent \textbf{Contributions.} We make four contributions.

\vspace{0.02in}\noindent
1) We contribute a characterization and analysis of the state-of-the-practice of experimentation with DNN4SE by addressing a fundamental question: \textbf{RQ1: To what extent are DNN4SE  experiments specified in papers?}
%\item[RQ2.] Do artifacts improve the specifications of these experiments? %(Section~\ref{sec:analysis_artifacts}). 
%\item[RQ3.] What are the implications of the current descriptions in the validity of the experimental findings? %(Section~\ref{sec:issues}).
%\end{itemize}
To answer that question, in Section~\ref{sec:analysis_papers}, we present a systematic analysis of 55 papers from ICSE, FSE, and TSE from 2018-2021 that apply DL techniques to automate SE tasks. Building on 
a cause-effect model of the experimental space and the variables relevant to DNNs, we determine the degree to which the variable space in the experiments was specified by each paper. 
We find that while most papers clearly identify, for example, the response variables (76\%) and training data (70\%), none describe their complete space of variables. Furthermore,  most papers lack in critical  aspects like the choice for experimental design  to control the sources of variability (30\%) and the use of even descriptive statistics as part of the results analysis and interpretation (56\%). This lack of specificity is not just an under-reporting issue, but it  reflects a limited consideration of fundamental experimental aspects that threaten the validity of the findings. %\sv{I am not sure the values that correspond to A, B and C, as they are not single rows in Table 3, but groups of rows (e.g. variables identification has 5 rows.}

\vspace{0.02in}\noindent
2) Given the community ongoing efforts for sharing artifacts~\cite{artifactsInSE}, it seems reasonable to ask a follow-up question:
%whether the missing portions of the specifications are shared through artifacts. 
\textbf{RQ2. Do shared artifacts improve the specifications of DNN4SE  experiments provided in the papers?} To contribute an answer to this question, in Section~\ref{sec:analysis_artifacts}, we present an analysis of the artifacts   associated with the subset of papers that earned ACM artifact badges, increasing the scope of  analysis to include code, data, and documentation.  As expected, we find that the artifacts tend to provide complementary details about the experiments in the papers, especially about the definition of variables and the training and test data, all of which are necessary to operationalize the experiments. However, our analysis also reveals 
%that \se{x  of y experiments} 
%\sv{We need to be consistent throughout the section. Are we going to mention percentages or number of experiments out of total?}\se{Maybe stick to percentages in abstract and intro to give overall picture} 
%point to elements that are not accessible (e.g., data is missing, broken links, permission issues). 
%Even more important, 
that 68\% of the experiments reported in the artifacts present inconsistencies when compared with the corresponding paper, ranging from the loss function  to the testing data being used.  This is problematic because the additional effort invested   to prepare artifacts  to further support the experiments often raises doubts about which portions of the papers and the artifacts  are to be trusted. %\sv{Isn´t the 'neither' too strong?}.

%\vspace{0.05in} \noindent \textbf{Implications.} 
\vspace{0.02in}\noindent
3) \textbf{RQ3. What are the implications of the previous findings about the under-specification of DNN4SE experiments?} Section \ref{sec:issues} contributes the key implications   worth the attention of the community. First, by failing to clearly define factors and treatments, it is unclear whether the experimental results are caused by the intended constructs or by other variables that were not operationalized correctly. In the best of cases, one could argue that those unspecified  variables in the papers are controlled when the experiments are performed. However,  our analysis of artifacts reveals that that is rarely the case.
%, and it introduces the additional concern because of the inconsistencies found between artifacts and papers.
%, and the cross-papers analysis shows that  when other researchers consume  results from ambiguous experiments they introduce additional noise into their findings. 
%\se{did we do this last study? do we have data on it? If not, drop the last line} \sv{Yes, we do have data}\se{to drop} 
Second,   even variables are specified it is often unclear how they are controlled to  establish causality. We find that 
%less than \hl{1\%} of the experiments explicitly control for any kind \se{@sira: 1\% any kind? some control for some kind? check} of source of randomness, 
62\% \se{@Sira: of experiments?} account for sources of randomness related to the dataset, and none \se{@Sira: is it none or only one?} controlled for other sources of training randomness  by, for example, performing multiple training runs or varying the DNN initial weights. 
%In other words, 
%all experiments analyzed train the DNN only once for a single combination of hyperparameters. 
Third, we find that 52\% of experiments identify relationships between independent and dependent variables based on single observations which is suspect as it ignores any experimental fluctuation.
%, while 31\% identify relationships based on means which is stronger than single observations but without considering variance so the significance of the results is still doubtful.  

 \vspace{0.02in}\noindent \se{new paragraph - check carefully}
4) 
%\se{I think we need a small paragraph about recommendations here, right? Since we have one for studies and another for implications, it seems like we should since that is the fourth contribution.} \sv{Agree. But should be really short. We do not have space.}
The last contribution is a set of actionable
%\sv{basic? If they help alleviate concerns with half of the experiments only} 
recommendations (Section \ref{sec:recommendations}) for conducting and specifying DNN4SE experiments that, if adopted, would   alleviate the concerns with at least \se{half?} of the  experiments we analyzed. The recommendations include simple practices to control for common sources of randomness in DNN4SE,  increase the number of observations to perform more meaningful comparisons that account for experimental variability in DNNs, and  standardize a minimal specification and provide partial automation for synchronizing the paper and artifact content. 

\sv{I do not understand how you are measuring this (referring to the half above.} 
\se{It would be good to have a solid number, I just picked more than half because by having multiple runs we will be able at least   move from single-point comparisons (56\% of the experiments do that) to comparison of means. But if there is a more precise way to do it that would be great. @Sira was going to think about this more to see if we could give an exact number, hopefully a bigger one :)}
% \se{recheck once we complete once we finish implication section}
%\sv{Potential RQs in case we want to add some: \\
%    RQ1: To what extent are experiments described? \\
%        RQ1.1. Based on papers? \\
%        RQ1.2: Based on artifacts? \\   
%    RQ2: What are the implications of the current descriptions?\\
%	    RQ2.1: Is there a relationship between response variable and factor(s)? \\
%	    RQ2.2: Are the identified relationships causal? \\
 %       RQ2.3: Is the causal relationship real (true)? Do the experimental variables correctly implement the conceptual variables? 
%}

%\se{Minor TODO: replace `deep learning' for 'DL' in the rest of the paper}


%\se{What are we providing that those checklists are not? Are our datasets of programs and tests for example unique in some way that require special curation? or perhaps require new architectures to deal with multi-modal data? Or is it our contribution really just stating our the work in our community measures against those checklists? Talk to @Sira about this.}
%\se{Sira's answer: formalization and extension of the checklist}
%\se{Sira's answer: architectures are not novel, but one wonders whether some of the chosen architectures are appropriate}
%\se{Sira's answer: data and data cleaning/wrangling are unique because problem is unique, and so is the type of output we look at. @Sira: mentioned that some of the papers argue that the datasets are small}
%\sv{Lionel's slide and Gil's comment about code repository.}
%\se{Good point, I am keeping those in mind and still thinking about this tricky paragraph}

%\sv{@Sebastian. I am missing the research method. Discuss if it should appear in the introduction, or should be a separate section.} \se{Yes, acknowledged -- once we settle on the process, we will come back here to complete it}

%\se{Make sure to highlight the finding that the issues is not just that the experiments are poorly reported, but really poorly conducted}
 
%The contribut 


%\se{WE can also point to the Survey paper of DNN4SE which advocates for more ``rigorous research methodology to drive the scientific process'' as inspiration or as positioning this work}

==> sections/appendices.tex <==
% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%


\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


==> sections/background.tex <==

\section{Background}
\label{sec:background}

\sv{@Sebastian. Should DNNs go first?}

We provide a brief background on experimentation principles and neural networks, highlighting the key elements on which we will build later in the paper. 


\se{Throughout this section it would be good to go back to the motivating example, explaining what each term of the experiment definition in 2.1 means in terms of that example and what each part of the sample DNN maps to the DNN concepts introduced in 2.2}


\subsection{Brief Introduction to DNNs}

\subsection{Foundations of (SE?) Experimentation}
\label{sec:experiments}

An experiment~\cite{juristo2013basics} is an empirical procedure where key variables of a reality are manipulated in a controlled environment to investigate the impact of such variations over the response variable.
From this definition, we can infer three fundamental features in experiments: independent variable manipulation, minimization of the variability not associated to treatments, and statistical analysis. 

\textbf{Independent variable manipulation} (or treatment design), consists of choosing the variables that will be intentionally varied during the experiment~\cite{juristo2013basics}. 
%Independent variables (or factors) are the focus of the investigation~\cite{kuehl2000design}.
	
\textbf{Minimization of  variability not associated to treatments}. Ideally, the only source of variation in an experiment should be the one due to the manipulated variables. In practice, there is variation among identically and independently treated experimental units. This variation is called \textit{experimental error}~\cite{kuehl2000design}. Experimental design aims at minimizing the experimental error and its variance, and it has three fundamental components~\cite{kuehl2000design}: 


\se{I think we need to rework the following classification to better highlight the pieces that we will be working on later. Perhaps some of the actions under Local Control should be their own categories. Also It would be useful to get concise terms for all of this, a fixed vocabulary, so that we can later define the template using those terms}
\talk{@Sebastian: Can you be more precise? I am aware that although local control, replication and randomization are set at the same \say{level}, they have different degrees of complexity. But this is how the experimentation literature establishes its three pillars. Having said that, I am more than willing to change this :).}

\begin{itemize}


	\item Local control: Describes the actions an investigator employs to reduce or control experimental error, and therefore increase the accuracy of observations. \talk{@Sebastian: Maybe (re)move from here on?}Such actions include 1) the definition of an experimental protocol to guarantee that experimental tasks are performed uniformly throughout the experiment~\cite{kuehl2000design}, 2) the selection of experimental units that are as uniform as possible~\cite{kuehl2000design}, 3) the management of other variables by holding them constant, block them and measure them~\cite{montgomery2019design}, and 4) the design selection to assign treatments to units 	\cite{wohlin2012experimentation}.
	 

	\item Replication.  It consists of an independent repeat run of each factor combination~\cite{montgomery2019design} to estimate  the experimental error variance~\cite{kuehl2000design}. 

	\item Randomization. Allows a valid estimation of experimental error variance. Used for uncontrolled variables for which we assume relatively small effects~\cite{montgomery2019design} or that are unknown (ref. libro observational studies). \se{I am confused. Isn't randomization a key piece of the design as units are assigned to treatments? Isn't a way to control error (not estimate it)?} \talk{@Sebastian: Not exactly. It is a way to make that the part of the error that you cannot control is not biased. The assumption is that there is part of the error that cannot be controlled (cannot be addressed in local control), and all you can hope is that it is not biased. Note that you do this with unknown variables or variables with very little influence.}


\end{itemize}


\textbf{Statistical analysis} \se{I think we want to define what it is before stating what is necessary} is necessary if we wish to draw meaningful conclusions from the data~\cite{wohlin2012experimentation} \talk{@Sebastian: Will a footnote be enough or do you want it in the main text?}. When the experiment involves data that are subject to experimental errors, statistical methods are the only objective approach to analysis~\cite{montgomery2019design}. Statistical analysis is closely related to experimental design, as the statistical method to be used for analysis depends directly on the design chosen.

In this paper we will focus on comparative experiments. \se{This seems premature, why do we need to say this here?} \talk{@Sebastian. I have probably received too many times a comment saying \say{you should state this early in the paper :) When do you think we should mention it? Perhaps research method?}} There is more than one treatment, which are compared with one another~\cite{kuehl2000design}.

Figure~\ref{fig:experimental_process} shows the experimental process as described in~\cite{wohlin2012experimentation}. It consists of five phases: experiment scoping, planning, operation, analysis and interpretation, and presentation and packaging. \se{Why do we need this figure? What is it going to add besides that is in the text?} \talk{@Sebastian: I do not think that we need it. But since I had already placed it, I was afraid to remove it without having your opinion. This is the reason why I removed the figure and only left the caption.}

\talk{@Sebastian: I am missing here a link between the \say{three fundamental features} and the experimental process.}

\begin{figure}[h]
  \centering
%  \includegraphics[width=\linewidth]{figures/experiment_process}
  \caption{The experiment process (ref.).}
% \Description{A woman and a girl in white dresses sit in an open car.}
  \label{fig:experimental_process} 	
\end{figure}

\subsection{Neural Networks and Deep Learning}
\label{sec:NNs}

\sv{@Sebastian. NNs or DNNs? Now I am being inconsistent throughout the paper.}

\se{Should the background point to Fig2 to help with the description? It seems like a natural progression from left-to right, and a great visual walkthrough}
\talk{@Sebastian. I was afraid that it is too detailed. But if you think it would fit here, I will reference it.}

\se{This discussion is good, but I wonder whether we need to formalize it a bit, introducing the terms as variables that later on we can refer concisely when we defined our template. Something like the following (plagiarized from an older paper of mine  -- need to adjust). The key point is to introduce the terms that we will be using later in the other sections, like a domain-specific language or grammar for the domain }

\se{A DNN, N, is a type of machine learning model that is trained to approximate a partial target function $f : R_n \rightarrow R_m$. For example, f may classify some n-dimensional input (e.g., an image) as one of m possible classes (e.g., a digit in the range 0 to 9). f is partial in the sense that it is trained to generalize to a target data distribution, $D \in R_n$. 

DNNs are comprised of layers, $l_0 , ..., l_k$ , each of which performs some computation on their input (e.g., matrix multiplication or convolution). A typical linear architecture defines a DNN as the composition of layers, $N = lk ◦···◦l1 ◦l0$. Layers are comprised of neurons. The input of a neuron is defined as the weighted sum of the outputs of a set of neurons in a preceding layer where the connections between neurons have trainable parameters. The output of a neuron applies a non-linear activation function to the input.

Training involves initializing the parameters and then applying N to samples, (x, y), from the training set, T , and repeatedly updating parameters based on $\mid N(x)-y \mid$. The  goal of training is to learn the partial function f defined over D, D is generally unmanageably large (e.g., the set of road images visible on a forward facing camera). Consequently, the training set is defined as a representative sample of the data distribution, $T \sim D$. A well-trained network is said to generalize to the data distribution}


Machine learning (ML) is a subfield of Artificial Intelligence (AI) that enables computers to learn from experience (ref. Mitchell, Bengio). ML algorithms build a model based on sample (training) data  to make predictions or decisions without being explicitly programmed to do so (ref?). Deep Learning (DL) is a specific kind of ML with Deep Neural networks (DNNs) (ref libro intro, Bengio). 

\sv{Reducir.} NNs simulate the mechanism of learning in biological organisms (ref. NN\&DL). They consist of neurons, which are connected, and grouped in layers. There is always an input layer (that merely accepts inputs) and an output layer. Additionally, one or more \say{hidden} layers may exist between the input and output layer. A DNN has of two or more hidden layers, otherwise it is considered \say{shallow}. \sv{Quitar? In feedforward NNs, every neuron of a layer is connected to all neurons of the next layer, but neurons of the same layer are not interconnected.} Every connection between 2 neurons has a weight which regulates how much of the initial value will be forwarded to a given neuron. Each neuron has an associated value, called the \textit{bias}. 

The output of a network is computed as the sum of the products of the inputs nd respective weights, plus the bias. Additionally, a nonlinear function (called activation function) can be applied to the logit. All neurons in the same layer must have the same activation functions, although different layers may have different ones. 

This way, the flow of information goes from the first layer neurons, through the successive hidden layers to the output layer. A forward pass is the set of calculations that take place when the input travels through the NN to the output.

NNs need to be trained before they can be used. \textbf{Training} a NN consists of (ref. Bengio) adjusting its \textit{parameters} (weights and biases), using a \textit{DL} algorithm controlled by a set of \textit{hyperparameters} (training and model), using a \textit{dataset}. It is performed via backpropagation---the reverse of a forward pass. The error the network makes when calculating the output is measured, and backpropagated using gradient descent\footnote{Gradient descent is a first-order iterative optimization algorithm for finding a local minimum of a differentiable function (ref.).} to modify the weights (and biases?) so that this error becomes very small. 

\textbf{Datasets} are collections of examples (datapoints). Two types of datasets are used for training: training and validation (80\% and20\% of examples respectively \se{this is just a guideline, right? it is often different than that}) validation set test set. They are used to estimate the training error. If they are small, cross-validation is typically used\footnote{Repeat the training and testing computation on different randomly chosen subsets or splits of the original dataset.}. A test set is used to check how well the ML algorithm performs on data that it has not seen before. The test set is separate from training data, as it is intended to estimate the generalization error.

\textbf{Hyperparameters} are parameters that cannot be learned: either because it is impossible \se{why?} or because they choose the maximum possible model capacity, resulting in overfitting. They can be classified as model hyperparameters (refer to the model selection task) and training hyperparameters, that in principle have no influence on the performance of the model but affect the speed and quality of the learning process (such as number of epochs, batch size or number of iterations).

Nearly all \textbf{DL algorithms} can be described as a combination of (ref. Bengio): the specification of a dataset, a cost function, an optimization procedure and a model.

A ML algorithm has a good performance if it makes: the training error small, and the gap between training and test error small. \textbf{Regularization} techniques are strategies explicitly designed to reduce the generalization (test) error, possibly at the expense of increased training error (ref. Bengio). These include: parameter norm penalties, dropout, data augmentation, early stopping, etc.

\textbf{Optimization}. Finding the parameters (weights and biases) of a neural network that significantly reduce a cost function. Typically includes a loss function as well as additional regularization terms. Optimization is a extremely difficult task. Algorithms can be used, or parameter initialization strategies (no consensus of which one to use).

\sv{Mention other architectures: Convolutional and recurrent. Others? Check with @Sebastian.}

\sv{Discuss application of DNNs to SE.}

==> sections/biographies.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}{Sira Vegas}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiography}{Sebastian Elbaum}
Biography text here.
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% if you will not have a photo at all:
%\begin{IEEEbiographynophoto}{Jane Doe}
%Biography text here.
%\end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

==> sections/discussion.tex <==

\section{Recommendations}
\label{sec:recommendations}

\se{A few ideas for potential recommendations.} \sv{Should this be a summary of the recommendations given in the previous section?}

\begin{itemize}

    \item Complete our factor template. 
    Do not assume defaults as they may change across frameworks and even versions of frameworks. Do not assume something is known because deep learning is evolving rapidly and  assumptions do not hold for long. 
    \item An under-specified template means that the reported results constitute one out of a range of potential results.

    \item Share and maintain. As much as possible. Ongoing challenge for community to find the right mechanisms and support to curate and share gigantic datasets.
    
    \item Set up competitions but with enough evolution to avoid over-fitting a benchmark. Need to incentivize companies to run this competition. It is happening in other fields (Waymo, Uber, Lyft have large datasets for the perception community to refine their approaches)
    
    \item Include more SE context. Just applying a deep learning technique to a dataset is not solving an SE relevant and rich SE problem. 
    
    \item Do not blindly clone an experiment with a DNN
    
\end{itemize}


==> sections/removed_text.tex <==


\subsection{Operationalization of Response Variables} 

sv{Also take into consideration the conclusion validity threat about restriction and range.}

\se{@Sira: As per discussion, this does not seem like a major issue so I would comment this one out -- we could include it in an extended version of the paper in the future}

The response variables are mostly not directly measurable and they have to be measured via an indirect measure instead. As a consequence, the measure will affect the result of the experiment~\cite{wohlin2012experimentation}. The choice of the response variables also means that the metrics used and the measurement procedure followed have to be determined~\cite{gomez2014understanding}. For example, in the experiments associated to RQ1 and RQ2 in  (ref. paper 23), the authors describe that NN performance is measured by means of accuracy, precision, recall and F1, and it can be deduced that the measurement procedure followed consists of implementing the formulas given in the paper in the code.

Most of the experiments reported in our literature survey (80\%) fully address the operationalization of the response variables. Those few papers that do not do it is due to either a proper definition of the metrics used (the name of the metric is given along to a reference) or lack from definition at all (only the name of the metric is given). Although most of the experiments do not explicitly mention the measurement procedure, it can easily be deduced.

Since most of the experiments do properly deal with this aspect, we will only focus on two construct validity threats related to the response variables and specific metrics that are used to measure the response variable, which we believe the authors should take into consideration: \sv{@Sebastian, again, I am not sure if this is interesting for ICSE.}

\begin{itemize}

    \item\textit{Restricted generalizability across constructs}. The operationalization of a response variable may have \say{unintended consequences}. An experiment shows that a NN is more effective than others in terms of precision or recall. But the experiment does not anticipate that the performance of the network is much worse in terms of time. It is important to have in mind that observed effects do not necessarily generalize to other potential outcomes.
    
    \item\textit{Mono-method bias}. Sometimes, using a single metric is not enough to provide evidence that you are really measuring your response variable. As an example, most of the papers we have surveyed used both precision and recall to measure accuracy. This helps to tackle the mono-method validity threat. However, it is important to have in mind that when we define multiple metrics to measure the same construct, there is a risk that the fishing and the error rate threat to conclusion validity may become too large~\cite{wohlin2012experimentation}. \\
    
\end{itemize}

\noindent\framebox{%
\begin{minipage}{0.97\linewidth}
\textbf{Practical recommendation:} \newline
Describe the metric(s) used to measure the response variable and the measurement procedure that has been followed. Have in mind that your results cannot be generalized to other metrics and/or response variables. Try not to use too many metrics to measure the same respone variable.
\end{minipage}}



\subsection{Analysis and Interpretation}


\se{The following seems generic and not as relevant given that most paper did not even perform a statistical analysis. I would rather put the focus on emphasizing the problem and consequences of having just means, or having just box-plots which is what we see in the best case}

\begin{itemize}

    \item \textit{Low statistical power\footnote{Probability that a statistical test will reject the null hypothesis when it is false (ref.).}}. Mean and effect size estimates will be less precise (have wider confidence intervals) and traditional NHST may incorrectly conclude that there is no relationship between the response variable and the factor(s). This will happen if non-parametric tests are used when data meet the assumptions for using parametric tests, as non-parametric tests are less powerful. For example, in (ref.  paper X), the authors perform non-parametric tests without having checked whether parametric tests can be used.
    
    \item \textit{Low statistical power}. An insufficient powered experiment may incorrectly conclude that the relationship between treatment and outcome is not significant. It is necessary to set a high enough number of replications (this issue is discussed in \cite{arcuri2011practical}). All our papers are an extreme situation of low statistical power, as they work with just one replication. For example, \sv{Complete}.

    \item \textit{Violated assumptions of statistical tests}. Some statistical analysis techniques have assumptions about the nature of the data (e.g. normality of data or residuals). If you do not check the assumptions of the analysis technique you are using, you are likely to draw erroneous conclusions about results. \sv{@Sebastian, for the moment, no single paper suffers from this threat, because all papers I have read so far, use non-parametric tests. I am keeping this in case there is a paper of the pending ones that does suffer from this threat.} For example, in the experiment reported in (ref. paper X)... \sv{Either add an example, or remove the threat.}

    \item \textit{Fishing and the error rate problem}. Repeated tests for significant relationships, if uncorrected for the number of tests, can artifactually inflate statistical significance of an effect. This happens when the experiment has more than two treatments and multiple comparisons are performed over them, or multiple response variables are used in the experiment. For example, in experiment (ref. paper X), 3 response variables are measured, and no correction is used for the statistical tests used.
    
    \item \textit{Inaccurate effect size estimation}. Some effect size estimates (e.g. Cohen's d or Hedges' g) depend on the assumption that studies are normally distributed and have equal variance, and their value tends to be biased when these assumptions are not met~\cite{borenstein2011introduction}. \sv{Not sure if there will be an example for this, as nobody calculates the effect size. But there are examples where the mean difference is used (means comparison). We could point out that this is not a good effect size estimator.}
    
\end{itemize}




==> sections/table_artifacts.tex <==
 


  \begin{table*}[hbt]
  \caption{Characterization of (44) experiments that earned ACM Artifact Badges. Cells with a single label mean the artifact does not improve the information provided in the paper. Cells with an arrow mean that the information provided in the artifact improves the information provided in the paper. Light gray background represents an inconsistency between the content of the paper and the artifact. Dark gray background represents inconsistencies within the elements in the artifact.
  %(pdf supplementary material and code, or code with commented lines showing different options, none of them appearing in the paper).
  }
  
%  \se{On Table 5: 1) with an arrow when something gets better, 2) gray background where there is an inconsistency, 3) cell with a single label if nothing changed}
 
  \label{tab:artifacts}
  \scriptsize
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{lccccccccccccccc}
    \toprule
    	&	&	Hyp.	&	\multicolumn{5}{c}{Variables identification} & \multicolumn{2}{c}{Operationalization} &	\multicolumn{2}{c}{Design} 	&	Objects sel. 	&	\multicolumn{2}{c}{Analysis \&  interpr.} 			&	Val. eval.	\\		\cmidrule(lr{0.5mm}){3-3} \cmidrule(lr{0.5mm}){4-8} \cmidrule(lr{0.5mm}){9-10} \cmidrule(lr{0.5mm}){11-12} \cmidrule(lr{0.5mm}){13-13} \cmidrule(lr{0.5mm}){14-15} \cmidrule(lr{0.5mm}){16-16}
					
    
	&   	&	 Res.	&	Model 	&	Model 	&	DL 	&	Training 	&	Training 	&	 Factors   	&	 Resp.   	&	 Choice	&	 Instrum.	&	 Test set	&	Descr.	&	 Infer.	&	 Validity 	\\	
	
	&	   	&	 hyp.	&	hyper. 	&	params. 	&	alg. 	&	hyper. 	&	data 	&	 \& treat.  	&	 vars.   	&	 design	&	& chars.	&	stats.	&	 stats.	&	 threats 	\\						

	\midrule
	
\citeAP{paper22}	    &	E1	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M$\rightarrow$FA	&	PA	&	PA	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	& 	FA	 &	M	&	PA$\rightarrow$PA	&	M	&	M	&	M	&	M	\\
	    &	E2	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M$\rightarrow$FA	&	PA	&	PA	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	PA$\rightarrow$PA	&	M	&	M	&	M	&	M	\\
	    &	E3	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M$\rightarrow$FA	&	PA	&	PA	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	M	\\
	    &	E4	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M$\rightarrow$FA	&	PA	&	PA	&	FA	&	PA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	M	\\

\hline	    
	    
%&		&		&		&		&		&		&		&		&		&		&		&		&		&		&		\\	    

\citeAP{paper26}	    & E1		&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA	& \cellcolor{lightgray}FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	M	&	PA	&	PA	&	M	&	M	&	PA	\\
	    &	E2	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	M	&	PA	&	PA	&	M	&	M	&	PA	\\
	    &	E3	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	M	&	PA	&	PA	&	M	&	M	&	PA	\\
	    &	E4	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	M	&	PA	&	PA	&	M	&	M	&	PA	\\

\hline	    
	    
%&		&		&		&		&		&		&		&		&		&		&		&		&		&		&		\\	    

\citeAP{paper30}	    &	E1	&	M	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	PA$\rightarrow$FA	&	FA	&	PA$\rightarrow$PA	&	M$\rightarrow$FA	& PA	&	PA	&	PA	&	M	&	M	    &	PA	\\
	    &	E2	&	FA	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	PA$\rightarrow$FA	&	FA	&	PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	PA	&	FA	&	FA	    &	PA	\\
	    &	E3	&	FA	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	PA$\rightarrow$FA	&	FA	&	PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	PA	&	FA	&	M	    &	PA	\\
	    &	E4	&	FA	&	PA	&	M	&	PA	&	PA	&	FA	&	FA	&	FA	&	PA	&	PA	&	PA	&	FA	&	M	    &	PA	\\
	    
\hline	    
	    
%&		&		&		&		&		&		&		&		&		&		&		&		&		&		&		\\	    	  
	    
\citeAP{paper62}	    &	E1	&	FA	&	PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	PA	&	M	&	PA	\\
	    &	E2	&	FA	&	PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	PA	&	M	&	PA	\\
	    &	E3	&	FA	&	PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	PA	&	M	&	PA	\\

\hline	    
	    
%&		&		&		&		&		&		&		&		&		&		&		&		&		&		&		\\	    
	    
\citeAP{paper34}	    &	E1	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	PA$\rightarrow$FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}PA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	PA	&	PA	&	PA	&	PA	&	M	&	M	\\

\hline	    
	    
%&		&		&		&		&		&		&		&		&		&		&		&		&		&		&		\\	    

\citeAP{paper82}	    &	E1	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	\cellcolor{lightgray}FA	&	PA	&	PA	&	M	&	M	\\
	    &	E2	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA$\rightarrow$FA	&	\cellcolor{lightgray}PA	&	FA	&	M	&	\cellcolor{lightgray}FA	&	PA	&	M	&	M	&	M	\\
	    &	E3	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA$\rightarrow$FA	&	FA	&	M$\rightarrow$FA	&	M	&	\cellcolor{lightgray}FA	&	PA	&	M	&	M	&	M	\\
	    &	E4	&	FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}FA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	PA	&	M	&	M	&	M	\\
	    
\hline	    
	    
%&		&		&		&		&		&		&		&		&		&		&		&		&		&		&		\\	    

\citeAP{stateformer}	    &	E1	&	FA	&	\cellcolor{gray}FA	& M	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}PA	&	FA	&	PA	&	\cellcolor{lightgray}PA	&	FA	&	M	&	M	&	PA	\\
	    &	E2	&	FA	&	\cellcolor{gray}FA	&	M	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}PA	&	FA	&	PA	&	\cellcolor{lightgray}PA	&	FA	&	PA	&	M	&	PA	\\
	    &	E3	&	FA	&	\cellcolor{gray}FA	&	M	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}PA	&	FA	&	PA	&	\cellcolor{lightgray}PA	&	FA	&	PA	&	M	&	PA	\\
	    &	E4	&	FA	&	\cellcolor{gray}FA	&	M	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}PA	&	FA	&	PA	&	\cellcolor{lightgray}PA	&	FA	&	PA	&	M	&	PA	\\
	    &	E5	&	FA	&	\cellcolor{gray}FA	&	M	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}PA	&	FA	&	PA	&	\cellcolor{lightgray}PA	&	FA	&	PA	&	M	&	PA	\\
	    &	E6	&	FA	&	\cellcolor{gray}FA	&	M	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}PA	&	FA	&	M	&	\cellcolor{lightgray}PA	&	FA	&	M	&	M	&	PA	\\
	    &	E7	&	FA	&	\cellcolor{gray}FA	&	M	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}PA	&	FA	&	M	&	\cellcolor{lightgray}PA	&	FA	&	M	&	M	&	PA	\\
	    &	E8	&	FA	&	\cellcolor{gray}FA	&	M	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}PA	&	FA	&	M	&	\cellcolor{lightgray}PA	&	FA	&	PA	&	M	&	PA	\\
	    &	E9	&	M	&	\cellcolor{gray}M$\rightarrow$FA	&	M	&	M$\rightarrow$FA	&	M$\rightarrow$FA	&	\cellcolor{gray}M$\rightarrow$FA	&	M$\rightarrow$FA	&	M$\rightarrow$PA	&	M	&	\cellcolor{gray}M$\rightarrow$PA	&	M$\rightarrow$FA	&	M$\rightarrow$PA	&	M	&	M	\\
	    &	E10	&	M	&	\cellcolor{gray}M$\rightarrow$FA	& M	&	M$\rightarrow$FA	&	M$\rightarrow$FA	&	\cellcolor{gray}M$\rightarrow$FA	&	M$\rightarrow$FA	&	M$\rightarrow$FA	&	M	&	\cellcolor{gray}M$\rightarrow$PA	&	M$\rightarrow$FA	&	M	&	M	&	M	\\
	    &	E11	&	M	&	\cellcolor{gray}M$\rightarrow$FA	&	M	&	M$\rightarrow$FA	&	M$\rightarrow$FA	&	\cellcolor{gray}M$\rightarrow$FA	&	\cellcolor{gray}M$\rightarrow$PA	&	M$\rightarrow$FA	&	M	&	\cellcolor{gray}M$\rightarrow$PA	&	M$\rightarrow$FA	&	M	&	M	&	M	\\
	    &	E12	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}FA	&	M	&	FA	&	FA	&	\cellcolor{gray}FA	&	FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{gray}FA	&	FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}FA	&	\cellcolor{lightgray}FA	\\
	    

\hline	    
	    
%&		&		&		&		&		&		&		&		&		&		&		&		&		&		&		\\	    



\citeAP{syntaxguided}	    &	E1	&	FA	&	PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}FA	&	PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E2	&	FA	&	PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}FA	&	PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E3	&	FA	&	PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}FA	&	PA$\rightarrow$FA	&	PA	&	PA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E4	&	FA	&	PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}FA	&	PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$FA	&	\cellcolor{lightgray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E5	&	M	&	PA$\rightarrow$FA	&	M	&	\cellcolor{lightgray}FA	&	PA$\rightarrow$FA	&	PA	&	PA	&	FA	&	PA	&	PA	&	M	&	FA	&	M	&	PA	\\
	    

\hline	    
	    
%&		&		&		&		&		&		&		&		&		&		&		&		&		&		&		\\	    


\citeAP{lightweight}	    &	E1	&	M	&	PA	&	M	&	PA	&	PA	&	M	&	FA	&	M	&	M	&	M	&	M	&	M	&	M	&	PA	\\
	    &	E2	&	FA	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	\cellcolor{gray}PA$\rightarrow$FA	&	FA	&	\cellcolor{gray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E3	&	FA	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	\cellcolor{gray}PA$\rightarrow$FA	&	FA	&	\cellcolor{gray}PA$\rightarrow$PA	&	FA	&	M	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E4	&	FA	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	\cellcolor{gray}PA$\rightarrow$FA	&	FA	&	\cellcolor{gray}PA$\rightarrow$PA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E5	&	FA	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	\cellcolor{gray}PA$\rightarrow$FA	&	FA	&	\cellcolor{gray}PA$\rightarrow$PA	&	FA	&	M	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E6	&	M	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	\cellcolor{gray}PA$\rightarrow$FA	&	FA	&	\cellcolor{gray}PA$\rightarrow$PA	&	FA	&	M	&	PA	&	M	&	M	&	M	&	PA	\\
	    &	E7	&	M	&	PA$\rightarrow$FA	&	M	&	PA$\rightarrow$FA	&	\cellcolor{gray}PA$\rightarrow$FA	&	FA	&	FA	&	FA	&	PA	&	PA	&	M	&	M	&	M	&	PA	\\

\bottomrule
\end{tabular}
\end{table*}

